Unsupervised Disentanglement without Autoencoding: Pitfalls and Future Directions

Disentangled visual representations have largely been studied with generative models such as Variational AutoEncoders (VAEs). While prior work has focused on generative methods for disentangled representation learning, these approaches do not scale to large datasets due to current limitations of generative models. Instead, we explore regularization methods with contrastive learning, which could result in disentangled representations that are powerful enough for large scale datasets and downstream applications. However, we find that unsupervised disentanglement is difficult to achieve due to optimization and initialization sensitivity, with trade-offs in task performance. We evaluate disentanglement with downstream tasks, analyze the benefits and disadvantages of each regularization used, and discuss future directions.

==> semisup_exps.tex <==

\smallskip 
\noindent\textbf{Supervised Experiments}
Why we moved to semisupervised (as a result of unsupervised results) Note that we only use hessian variants for semi-sup and sup results since they were the best

tables of dsprites results

why supervision overpowers regularization
\begin{comment}
no reg semisup mnist stl10 xmanager exp ids
upstream: 22659978, 22659805, 22659994, 22659819, 22660006

downstream: 23040957, 23041156, 23041414, 23042353, 23042174, 23042661
23042641, 23042727, 23043668, 23044016, 23044539, 23044691
23081028, 23081049, 23081253, 23081487, 23081410, 23081423
23047687, 23047708, 23047890, 23047761, 23048112, 23047817
23080178, 23080231, 23080428, 23080547, 23080656, 23081160
\end{comment}
\begin{table*}[h]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Cls & \multicolumn{2}{c|}{0\%} & \multicolumn{2}{c|}{1\%} & \multicolumn{2}{c|}{5\% }& \multicolumn{2}{c|}{10\%} & \multicolumn{2}{c|}{100\%} \\ 
    \cline{2-11}
    Input & DC & BC & DC & BC & DC & BC & DC & BC& DC & BC\\
    \hline
         $z$ & 55.5 & 41.6 & 65.8 & 43.1 & 69.8 & 40.6 & 65.6 & 40.6 & 93.2 & 59.5 \\
         \hline
         $z_0$ & 41.4 & 31.2 & 52.0 & 32.1 & 41.5 & 26.3 & 45.8 & 26.6 & 75.0 &53.1 \\
         \hline
         $z_1$ & 32.6 & 31.3 & 50.6 & 26.8 & 38.5 & 27.0 & 42.9 & 26.7 & 62.2 & 53.1 \\
         \hline
    \end{tabular}
    \caption{semisup mnist stl10 no regularization}
    \label{tab:semihesse3}
\end{table*}

\begin{comment}
hessian xmanager exp ids
upstream: 22657917, 22658016, 22658022, 22657938, 22658125

downstream: 22750795, 22750879, 22750834, 22751008, 22750847, 22750819
22751096, 22751278, 22751263, 22751314, 22751208, 22751215
22751371, 22751257, 22751585, 22751410, 22751484, 22751379
22751451, 22751663, 22751707, 22751873, 22751732, 22751763
22754487, 22754498, 22754405, 22754507, 22754243, 22754342
\end{comment}
\begin{table*}[h]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Cls & \multicolumn{2}{c|}{0\%} & \multicolumn{2}{c|}{1\%} & \multicolumn{2}{c|}{5\% }& \multicolumn{2}{c|}{10\%} & \multicolumn{2}{c|}{100\%} \\ 
    \cline{2-11}
    Input & DC & BC & DC & BC & DC & BC & DC & BC& DC & BC\\
    \hline
         $z$ & 63.5 & 34.5 & 69.9 & 39.6 & 59.2 & 40.6 & 63.7 & 35.3 & 89.6 & 58.9\\
         \hline
         $z_0$ & 33.5 & 27.3 & 48.0 & 28.6 & 46.9 & 27.4 & 46.5 & 26.7 & 67.5 & 56.8 \\
         \hline
         $z_1$ & 40.4 & 24.1 & 51.1 & 30.7 & 45.3 & 33.4 & 48.7 & 27.8 & 64.2 & 56.8 \\
         \hline
    \end{tabular}
    \caption{semisup mnist stl10 hessian 1e-3}
    \label{tab:semihesse3}
\end{table*}

\begin{comment}
hessian xmanager exp ids
upstream: 22658141, 22658151, 22658764, 22658862, 22658774

downstream: 22755014, 22754532, 22754675, 22754554, 22754873, 22754894
22755033, 22755197, 22755463, 22755284, 22755251, 22755387
22755346, 22755445, 22755459, 22755591, 22755688, 22755697
22755991, 22755983, 22755906, 22755892, 22755632, 22755725
22756565, 22756467, 22756364, 22756045, 22756535, 22756142
\end{comment}
\begin{table*}[h]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Cls & \multicolumn{2}{c|}{0\%} & \multicolumn{2}{c|}{1\%} & \multicolumn{2}{c|}{5\% }& \multicolumn{2}{c|}{10\%} & \multicolumn{2}{c|}{100\%} \\ 
    \cline{2-11}
    Input & DC & BC & DC & BC & DC & BC & DC & BC& DC & BC\\
    \hline
         $z$ & 62.3 & 41.2 & 68.3 & 44.9 & 66.0 & 38.7 & 60.3 & 36.8 & 86.7 & 59.2 \\
         \hline
         $z_0$ & 39.8 &27.2 & 46.9 & 31.8 & 49.4 & 22.8 & 48.8 & 25.7 & 59.7 & 56.4 \\
         \hline
         $z_1$ & 48.2 & 29.2 & 41.5 & 28.2 & 41.2 & 33.0 & 52.7 & 24.9 & 58.4 & 57.0 \\
         \hline
    \end{tabular}
    \caption{semisup mnist stl10 hessian 1e-1}
    \label{tab:semihesse3}
\end{table*}
\begin{comment}
grad prod xmanager exp ids
upstream: 22657964, 22657881, 22657988, 22657980, 22658082

downstream: 22745972, 22745770, 22745909, 22745883, 22746266, 22745857
22746209, 22746232, 22746340, 22746465, 22746129, 22746383
22746785, 22746652, 22746962, 22746426, 22746509, 22746438, 
22746937, 22747047, 22746819, 22746830, 22746807, 22746987
22747501, 22747188, 22747219, 22747204, 22747469, 22747365
\end{comment}
\begin{table*}[h]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Cls & \multicolumn{2}{c|}{0\%} & \multicolumn{2}{c|}{1\%} & \multicolumn{2}{c|}{5\% }& \multicolumn{2}{c|}{10\%} & \multicolumn{2}{c|}{100\%} \\ 
    \cline{2-11}
    Input & DC & BC & DC & BC & DC & BC & DC & BC& DC & BC\\
    \hline
         $z$ & 46.7 & 39.7 & 72.6 & 44.7 & 69.2 & 43.3 & 60.3 & 40.5 & 88.6 & 59.9 \\
         \hline
         $z_0$ & 36.2 & 28.0 & 48.7 & 27.9& 45.8 & 30.6 & 39.8 & 28.4 & 57.3 & 57.9 \\
         \hline
         $z_1$ & 35.7 & 30.8 & 43.1 & 32.0 & 49.4 & 30.0 & 42.2 & 31.5 & 52.3& 57.4 \\
         \hline
    \end{tabular}
    \caption{semisup mnist stl10 grad prod 1e-3}
    \label{tab:semihesse3}
\end{table*}
\begin{comment}
grad prod xmanager exp ids
upstream: 22657428, 22657531, 22657442, 22657449, 22657860

downstream: 22745447, 22745625, 22745525, 22745483, 22745470, 22745374
22744352, 22744324, 22744324, 22743754, 22743425, 22743134
22744701, 22744614, 22744531, 22744684, 22744673, 22744576
22744883, 22744866, 22745060, 22744557, 22744736, 22744730
22744896, 22745108, 22745090, 22745132, 22745122, 22744953
\end{comment}
\begin{table*}[h]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Cls & \multicolumn{2}{c|}{0\%} & \multicolumn{2}{c|}{1\%} & \multicolumn{2}{c|}{5\% }& \multicolumn{2}{c|}{10\%} & \multicolumn{2}{c|}{100\%} \\ 
    \cline{2-11}
    Input & DC & BC & DC & BC & DC & BC & DC & BC& DC & BC\\
    \hline
         $z$ & 42.6 & 37.5 & 78.2 & 47.0 & 64.4 & 36.6 & 61.0 & 39.0 & 85.4 & 57.5 \\
         \hline
         $z_0$ & 32.6 & 26.8 & 48.7 & 33.8 & 42.5 & 25.7 & 40.9 & 26.8 & 56.9 & 55.1\\
         \hline
         $z_1$ & 32.3 & 32.0 & 42.9 & 31.5 & 39.3 & 27.7 & 41.9 & 25.4 & 61.3 & 54.0 \\
         \hline
    \end{tabular}
    \caption{semisup mnist stl10 grad prod 1e-1}
    \label{tab:semihesse3}
\end{table*}

\begin{comment}
no reg dsprites xmanager exp ids
upstream: 20802258

downstream: 20964526, 20964826, 20964722, 20964802, 20964414, 20964426
20955291, 20955404, 20955489, 20955396, 20955197, 20955021, 
20956756, 20956740, 20956652, 20956539, 20956442, 20956813
20959535, 20959623, 20959558, 20959841, 20960061, 20959732
20953947, 20954136, 20954030, 20954243, 20954360, 20954367
\end{comment}

\begin{table*}[h]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Cls & \multicolumn{2}{c|}{0\%} & \multicolumn{2}{c|}{1\%} & \multicolumn{2}{c|}{5\% }& \multicolumn{2}{c|}{10\%} & \multicolumn{2}{c|}{100\%} \\ 
    \cline{2-11}
    Input & S & O & S & O & S & O & S & O & S & O\\
    \hline
         $z$ & 43.5 & 7.5 & 64.4 & 7.6 & 90.2 & 18.1 & 92.3 & 30.2 & 99.0 & 64.6\\
         \hline
         $z_0$ & 43.5 & 7.5& 48.4 & 7.4 & 89.5 & 8.2 & 92.0 & 8.4 & 99.0 & 6.4 \\
         \hline
         $z_1$ & 43.5 & 7.4 & 46.0 & 7.5 & 43.4 & 14.6 & 37.7 & 29.2 & 36.2 & 64.6\\
         \hline
    \end{tabular}
    \caption{semisup dsprites no regularization}
    \label{tab:semihesse3}
\end{table*}
\begin{comment}
hessian 1e-3 dsprites xmanager exp ids
upstream: 20808281, 20808384, 20813357, 20813865, 20808120

downstream: 20964553, 20964654, 20964838, 20964892, 20965178, 20964991
20967628, 20967441, 20967525, 20967351, 20967634, 20967528
20969176, 20969278, 20968898, 20969090, 20968891, 20968815
20966811, 20966807, 20967093, 20966909, 20967103, 20967016
20965944, 20966171, 20965754, 20966470, 20966560, 20966563
\end{comment}

\begin{table*}[h]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Cls & \multicolumn{2}{c|}{0\%} & \multicolumn{2}{c|}{1\%} & \multicolumn{2}{c|}{5\% }& \multicolumn{2}{c|}{10\%} & \multicolumn{2}{c|}{100\%} \\ 
    \cline{2-11}
    Input & S & O & S & O & S & O & S & O & S & O\\
    \hline
         $z$ & 42.5 & 7.1 & 65.0 & 7.5 & 90.2 & 18.2 & 92.2 & 29.6 & 99.0 & 64.4\\
         \hline
         $z_0$ & 42.4 & 7.1 & 47.9 & 7.3 & 89.6 & 8.5 & 91.9 & 8.2 & 99.0 &12.0 \\
         \hline
         $z_1$ & 42.4 & 7.1 & 45.8 & 7.4 & 43.5 & 15.2 & 38.9 & 28.9 & 37.4 & 64.5 \\
         \hline
    \end{tabular}
    \caption{semisup dsprites hessian 1e-3}
    \label{tab:semihesse3}
\end{table*}
\begin{comment}
hessian 1e-1 dsprites xmanager exp ids
upstream: 20807609, 20807887, 20807531, 20807794, 20807809

downstream: 21052178, 21052112, 21052363, 21052118, 21052265, 21052267
21053167, 21052754, 21053109, 21053014, 21053107,21052929 
21060227, 21060480, 21060228, 21060240, 21060414, 21060497
21075616, 21075431, 21075418, 21075322, 21075663, 21075346
21077042, 21077138, 21077142, 21077055, 21077281, 21077199
\end{comment}
\begin{table*}[h]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Cls & \multicolumn{2}{c|}{0\%} & \multicolumn{2}{c|}{1\%} & \multicolumn{2}{c|}{5\% }& \multicolumn{2}{c|}{10\%} & \multicolumn{2}{c|}{100\%} \\ 
    \cline{2-11}
    Input & S & O & S & O & S & O & S & O & S & O\\
    \hline
         $z$ & 42.0 & 7.0 & 64.2 & 7.8 & 90.3 & 19.6 & 91.9 & 29.8 & 99.0 & 64.3 \\
         \hline
         $z_0$ & 42.1 & 7.1 & 50.6 & 7.6 & 89.7 & 8.5 & 91.8 & 7.9 & 99.0 & 5.8 \\
         \hline
         $z_1$ & 42.1 & 7.0 & 48.0 & 7.7 & 43.6 & 16.7 & 38.1 & 28.6 & 37.8 &64.3 \\
         \hline
    \end{tabular}
    \caption{semisup dsprites hessian 1e-1}
    \label{tab:semihesse3}
\end{table*}

\begin{comment}
grad prod 1e-3 dsprites xmanager exp ids
upstream: 21061019, 21061032, 21060951, 21061325, 23137149

downstream: 21107227, 21107052, 21107419, 21107821, 21107740, 21108090
21132878, 21133281, 21133172, 21133214, 21133011, 21132942
21134566, 21134371, 21134250, 21134059, 21134578, 21134474
21135293, 21135113, 21135593, 21135508, 21135310, 21135122
23145930, 23146043, 23146284, 23146494, 23146356, 23146671
\end{comment}
\begin{table*}[h]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Cls & \multicolumn{2}{c|}{0\%} & \multicolumn{2}{c|}{1\%} & \multicolumn{2}{c|}{5\% }& \multicolumn{2}{c|}{10\%} & \multicolumn{2}{c|}{100\%} \\ 
    \cline{2-11}
    Input & S & O & S & O & S & O & S & O & S & O\\
    \hline
         $z$ & 43.7 & 7.4 & 63.1 & 7.5 & 90.2 & 19.7 & 92.2 & 30.1 & 96.4 & 48.5 \\
         \hline
         $z_0$ & 43.7 & 7.4 & 48.1 & 7.2 & 89.6 & 7.7 & 91.9 & 8.5 & 80.0 & 27.9 \\
         \hline
         $z_1$ & 43.7 & 7.4 & 46.1 & 7.4 & 42.2 & 16.1 & 39.2 & 29.2 & 78.0 &25.3 \\
         \hline
    \end{tabular}
    \caption{semisup dsprites grad prod 1e-3}
    \label{tab:semihesse3}
\end{table*}

\begin{comment}
grad prod 1e-1 dsprites xmanager exp ids
upstream: 23138816, 21076497, 21076606, 21076554, 23139684

downstream: 23144960, 23144982, 23145119, 23144910, 23144939, 23145133
21151683, 21151449, 21151676, 21151423, 21151536, 21151692
21152333, 21152136, 21152237, 21152686, 21152250, 21152146
21166313, 21166227, 21166576, 21172083, 21172026, 21171831
23145563, 23145701, 23145621, 23145730, 23145879, 23145896
\end{comment}
\begin{table*}[h]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Cls & \multicolumn{2}{c|}{0\%} & \multicolumn{2}{c|}{1\%} & \multicolumn{2}{c|}{5\% }& \multicolumn{2}{c|}{10\%} & \multicolumn{2}{c|}{100\%} \\ 
    \cline{2-11}
        Input & S & O & S & O & S & O & S & O & S & O\\

    \hline
         $z$ & 50.0 & 6.7 & 62.5 & 7.3 & 90.4 & 17.2 & 92.4 & 30.1 & 98.0 & 56.0 \\
         \hline
         $z_0$ & 44.4 & 4.7 & 48.7 & 7.1 & 89.8 & 8.3 & 92.2 & 7.7 & 93.8 & 27.6 \\
         \hline
         $z_1$ & 43.4 & 4.8 & 46.6 & 7.2 & 44.3 & 14.7 & 39.2 & 29.3 & 83.2 & 25.3 \\
         \hline
    \end{tabular}
    \caption{semisup dsprites grad prod 1e-1}
    \label{tab:semihesse3}
\end{table*}
% but experiment 21042058 from before sync has similar losses to 23139684, so I don't understand
